Towards Automated Safety Coverage and Testing for Autonomous Vehicles with Reinforcement Learning

The kind of closed-loop verification likely to be required for autonomous vehicle (AV) safety testing is beyond the reach of traditional test methodologies and discrete verification. Validation puts the autonomous vehicle system to the test in scenarios or situations that the system would likely encounter in everyday driving after its release. These scenarios can either be controlled directly in a physical (closed-course proving ground) or virtual (simulation of predefined scenarios) environment, or they can arise spontaneously during operation in the real world (open-road testing or simulation of randomly generated scenarios). In AV testing, simulation serves primarily two purposes: to assist the development of a robust autonomous vehicle and to test and validate the AV before release. A challenge arises from the sheer number of scenario variations that can be constructed from each of the above sources due to the high number of variables involved (most of which are continuous). Even with continuous variables discretized, the possible number of combinations becomes practically infeasible to test. To overcome this challenge we propose using reinforcement learning (RL) to generate failure examples and unexpected traffic situations for the AV software implementation. Although reinforcement learning algorithms have achieved notable results in games and some robotic manipulations, this technique has not been widely scaled up to the more challenging real world applications like autonomous driving.

==> acknowledgments.tex <==
I am grateful to my advisor, professor Madhur Behl, whose support was inevitable during my MS program at UVA. Also, I thank the committee members, professors Sebastian Elbaum and Matthew Dwyer. In addition, I would like to thank Mārtiņš Možeiko and other members of the LGSVL, who provided much technological support on the simulator through GitHub. Most importantly, I would like to thank my parents.

==> intro.tex <==
Today, countless tech corporations and startups are investing billions of dollars to develop autonomous vehicles (AV). In fact, several businesses will deploy their vehicles in the next several years~\cite{timeline}. Alphabet's autonomous vehicle business, Waymo, recently announced that their commercial self-driving service, Waymo One, will begin to deploy fully driverless cars~\cite{techcrunch}.

The question then arises, "How safe are they?" Many AV companies use computer vision, a branch of machine learning, to learn the surroundings of the AV. They drive their AVs for billions of miles to try to observe as many of the combinations of such surroundings or scenarios. By doing so, when the AVs encounter a similar scenario in the future, they will know how to navigate safely through. However, due to the high number of both static and dynamic variables involved in driving, it becomes infeasible to perform safety coverage on every possible driving scenario.

Therefore, the kind of closed-loop verification likely to be required for AV component testing is beyond the reach of traditional test methodologies and discrete verification.
%There will remain some small risk of crashes. 
%The concept of residual risk has already been accepted for a long time now (see the rollout of airbags or new medicines). 
Validation puts the autonomous vehicle system to the test in scenarios or situations that the system would likely encounter in everyday driving after its release. 
These scenarios can either be controlled directly in a physical (closed-course proving ground) or virtual (simulation of pre-defined scenarios) environment, or they can arise spontaneously during operation in the real world (open-road testing or simulation of randomly generated scenarios).

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/agent.png}
    \caption{The reinforcement learning agent is tasked with the objective to maximize the reward associated with causing a collision for a given AV implementation. In this unique setting, the action space of the agent is the simulator/scene setup - i.e. the static and dynamic elements of the scene. After adequate iterations, the agent returns the scenario that is most likely to cause the AV to fail.}
    \label{fig:agent}
\end{figure}

 % For automotive applications, simulations may consider an entire system (e.g. a full vehicle with tires and automated driving system functions), a subsystem (e.g. an actuator or a hardware controller) or a component (e.g. a sensor or a communication bus).
In AV testing, simulation serves primarily two purposes: to assist the development of a robust autonomous vehicle and to test and validate the AV before release.
% In the case that model accuracy can be shown to sufficiently match real world behavior, simulation could conceivably be used to argue safety directly without real world driving activities. However, doing so would require a representative sample of simulation scenarios or a defensible mathematical expression for the contribution of each simulation scenario to the total statistical confidence in the system, likely based on the frequency of occurrence of scenarios in real-world driving.
A challenge arises from the sheer number of scenario variations that can be constructed from each of the above sources due to the high number of variables involved (most of which are continuous). 
Even with continuous variables discretized, the possible number of combinations becomes practically infeasible to test. 
To overcome this challenge we propose using reinforcement learning (RL)~\cite{sutton2018reinforcement} to generate failure examples and unexpected traffic situations for the AV software implementation. 
Although RL algorithms have achieved notable results in games and some robotic
manipulations, this technique has not been widely scaled up to the more challenging real world applications like autonomous driving.

The frame of RL is an agent learning through interaction with its environment driven by an impact (reward) signal. The environment reinforces the agent to select new actions to improve learning process, hence the name of reinforcement learning~\cite{jaafra2018review}. 
RL algorithms have achieved notable results in many domains as games~\cite{mnih2015human,silver2016mastering} and advanced robotic manipulations~\cite{levine2016end, lillicrap2015continuous} beating human performance. However, standard RL strategies that randomly explore and learn lose efficiency and become computationally intractable when dealing with high-dimensional and complex environments~\cite{Wahlstrom2015FromPT}.
The origin of its difficulty lies in the important variability inherent to the driving task (e.g. uncertainty of human behavior, diversity of driving styles, complexity of scene perception, etc).

In our approach (Figure~\ref{fig:agent}), we rely on the LG Silicon Valley Lab (LGSVL) simulator~\cite{lgsvl}, a photo-realistic AV simulator that accepts scenario (or simulation) parameters through a Python API. 
For an input scenario, the API provides a way to vary the static (road geometry, position of traffic signs and lights, number of lanes, etc.) and dynamic parameters (weather, movement of other agents, pedestrians, etc.) of the simulator. The key insight is that the parameter space of the simulator, $\Psi$, is the action space for the reinforcement learning agent. 
For a given implementation of the AV software stack, such as Apollo from Baidu~\cite{fan2018baidu} or Autoware~\cite{kato2015open}, the agent's objective is to choose a set of simulation parameters (static and dynamic) such that it can cause the AV to fail. For each instance of the simulated scenario, the agent receives a reward if it can cause the AV to crash. Additionally, it receives a continuous reward to minimize a safety metric, such as time-to-collision.
The learned policy is a set of simulation parameters that could cause the AV to fail on the chosen safety metric. 
